An Interface Tracking Method with Triangle Edge Cuts

This paper introduces a volume-conserving interface tracking algorithm on unstructured triangle meshes. We propose to discretize the interface via triangle edge cuts which represent the intersections between the interface and the triangle mesh edges using a compact 6 numbers per triangle. This enables an efficient implicit representation of the sub-triangle polygonal material regions without explicitly storing connectivity information. Moreover, we propose an efficient advection algorithm for this interface representation that is based on geometric queries and does not require an optimization process. This advection algorithm is extended via an area correction step that enforces volume-conservation of the materials. We demonstrate the efficacy of our method on a variety of advection problems on a triangle mesh and compare its performance to existing interface tracking methods including VOF and MOF.

==> letter.tex <==
Dear Editor,

Thank you for your email regarding the major revision of our manuscript. In the revised version of the manuscript, we have addressed the grammatical errors and made vocabulary adjustments to enhance readability. Below is a summary of the changes made to correct the grammatical errors identified:

p4 
linear->nonlinear
sub-grid-accuracy -> sub-grid-accurate

p5
Shashkov and Kikinzon -> add names before cite

p7
geometry structure->geometric structure

p8
interpolation factor->interpolation factors
Either -> either

p9
e.g.->i.e.
in these basic cases -> on these basic cases

p10
case -> cases

p12
deal with this issue -> address these issues
simplifies the interface...as linear segments -> to linear segments

p13
dashed curves -> dashed curve

p15
remove superscript n+1
farthest -> is farthest
depends -> depend

p16
L2 -> L1
vt** -> vt***

p17
1,R31 -> 1-R31

p18
implies -> imply

p19
case -> cases

p21
happens -> occur
cost -> costs

p22
remove misplaced "The Table Title"
cost -> costs

p23
Intersections -> intersections

p24
effort -> efforts

p26
add missing "representation"

p27
are -> were

p28
velocities -> velocity components

p31
error -> errors
is -> are
difference -> differences

p37
caption in table 11 -> lowercase
was -> is

p38
surface reconstruction -> interface reconstruction

p40,41
Figure -> Figures

We have highlighted the changes made in the revised manuscript using red color as requested. We look forward to your feedback on our revised manuscript. Thank you for your consideration.

Best regards,
Authors
